Sorting Balls and Water: Equivalence and Computational Complexity

Various forms of sorting problems have been studied over the years. Recently, two kinds of sorting puzzle apps are popularized. In these puzzles, we are given a set of bins filled with colored units, balls or water, and some empty bins. These puzzles allow us to move colored units from a bin to another when the colors involved match in some way or the target bin is empty. The goal of these puzzles is to sort all the color units in order. We investigate computational complexities of these puzzles. We first show that these two puzzles are essentially the same from the viewpoint of solvability. That is, an instance is sortable by ball-moves if and only if it is sortable by water-moves. We also show that every yes-instance has a solution of polynomial length, which implies that these puzzles belong to in NP. We then show that these puzzles are NP-complete. For some special cases, we give polynomial-time algorithms. We finally consider the number of empty bins sufficient for making all instances solvable and give non-trivial upper and lower bounds in terms of the number of filled bins and the capacity of bins.

==> fpt.tex <==

In this section, we consider a general algorithm for the water sort puzzle.
We have an instance of the water sort puzzle consists of $n+k$ bins of capacity $h$ and $hn$ units 
in the first $n$ bins with the color set $\calC=\{1,2,\ldots,C\}$ satisfying $\msize{\calC}\le n$.
Then the following theorem claims that the sort puzzles can be solved in polynomial time if $n$ is fixed.

\begin{theorem}
\label{th:fpt}
Let $B=\{b_1,\ldots,b_{n+k}\}$ be an instance of the water sort puzzle.
Each bin has capacity $h$ and the size of the color set is $C$.
Then there is an algorithm that solves the decision problem of the water/ball sort puzzle in 
$O((C h^3 \max\{h,C\})^n)$ time.
\end{theorem}
\begin{proof}
In the initial state of the instance, let $\alpha_i=(c_{i,1},\ldots,c_{i,h})$ 
be the contents of the bin $b_i$ for each $i$ with $1\le i\le n$, and
$\alpha_{i}=\epsilon$ for each $i$ with $n+1\le i\le n+k$.
(That is, $c_{i,j}\in \calC$ for each $1\le i\le n$ and $1\le j\le h$.)

For each $\alpha_i=(c_{i,1},\ldots,c_{i,h})$, we define a set of indices $f_{i,1},f_{i,2},\ldots$ in the following recursive way:
We first define $f_{i,1}=1$. If $\alpha_i$ is monochrome, $f_{i,2}$ is not defined.
Otherwise, $f_{i,2}$ is defined by $f_{i,1}+\phi(\alpha_i,c_{i,f_{i,1}})$.
That is, we have $c_{i,1}=c_{i,2}=\cdots=c_{i,f_{i,2}-1}\neq c_{i,f_{i,2}}$.
If the sequence $(c_{i,f_{i,2}},\ldots,c_{i,h})$ is monochrome, $f_{i,3}$ is not defined.
Otherwise, we let $\alpha'_i=(c_{i,f_{i,2}},\ldots,c_{i,h})$ and 
$f_{i,3}$ is defined by $f_{i,2}+\phi(\alpha'_i,c_{i,f_{i,2}})$.
We repeat this process and obtain $f_{i,1},f_{i,2},f_{i,3},\ldots$, which give us the sequence of indices 
where the color changes at that index (comparing to the previous ones) in the sequence $\alpha_i$.

By the definitions, $\alpha_i$ can be represented by a string 
$c_{i,1}^{f_{i,2}-f_{i,1}} c_{i,f_{i,2}}^{f_{i,3}-f_{i,2}} c_{i,f_{i,3}}^{f_{i,4}-f_{i,3}}\cdots$.
For simplicity, we write $\alpha_i$ as $(c_{i,1};f'_{i,1},c_{i,f_{i,2}};f'_{i,2},c_{i,f_{i,3}};f'_{i,3},\ldots)$,
where $f'_{i,j}=f_{i,j+1}-f_{i,j}$.
As discussed in Observation \ref{obs:mono}, $\alpha_i$ is monotonically decreasing up to $\epsilon$ except the top elements.
Precisely, any water-move can change $\alpha_i$ in two different ways:
(1) It decreases $f'_{i,j}$ in the first pair $(c_{i,j};f'_{i,j})$ in the current $\alpha_i$ and
(2) it increases $f'_{i,j}$ in the first pair $(c_{i,j};f'_{i,j})$ in the current $\alpha_i$.
When $f'_{i,j}$ becomes zero in (1), 
we update $\alpha_i$ by removing this pair from the top of $\alpha_i$.
Once $\alpha_i$ becomes $\epsilon$, the bin $b_i$ becomes empty.
Since then, $b_i$ should be monochrome.
Thus we then can represent the contents of $b_i$ by a pair $(c_{i,1};f'_{i,1})$,
where $f'_{i,1}$ is the number of units of color $c_{i,1}$ in $b_i$.
(Note that we can represent the bins $b_i$ with $i>n$ in the same manner.)
In summary, the number of possible states of $\alpha_i$ in sorting is $O((C\cdot h)^h)$ 
for $1\le i\le n$ and $O(Ch)$ for $n+1\le i\le n+k$.
Here, we consider a data structure to represent a state of $\alpha_i$ with $1\le i\le n$.
By keeping a copy of the initial state as a table, 
each state of $\alpha_i$ can be represented by the current top index $f_{i,j}$ 
and the number of units of the top color of the current state which can larger than the initial state 
before $\alpha_i$ becomes empty. (We note the top color can be obtained from the table with index $f_{i,j}$.)
Once $\alpha_i$ becomes empty, we need the color and the number of units of the bin.
Therefore, each state of $\alpha_i$ can be represented by 
a pair $(f_{i,j},n_i)$, where $n_i$ is the number of the units of the top color before $\alpha_i$ becomes empty,
and a pair $(c_i,n_i)$ where $c_i$ is the (top) color after $\alpha_i$ becomes empty.
Therefore, the number of states of $\alpha_i$ is $O(\max\{h,C\}\cdot h)$.
For a bin $b_i$ with $n<i\le n+k$, the number of states is $O(C\cdot h)$.

We now consider a naive search algorithm that checks every reachable state from the initial state in the configuration space.
By above discussion, the size of search space is bounded by $O((\max\{h,C\}\cdot h)^n \cdot (C\cdot h)^k)$.
By discussion in Section \ref{sec:bins}, we can assume that $k\le C\le n$ without loss of generality for solving the decision problem.
%We also have $C\le n$.
Since each water-move can be applied in $O(h)$ time\footnote{It is not difficult to improve this 
time complexity $O(h)$ to $O(1)$, which is omitted here.} to update the states of target two bins,
the naive algorithm runs in $O((C h^3 \max\{h,C\})^n)$ time.
\end{proof}


==> poly.tex <==

% main.tex から 直接 h2 を読むようにしました

%In this section, we give two polynomial-time algorithms for the sorting puzzles.
%Since each water-move can be simulated by at most $h$ ball moves, we focus on the water sort puzzle in this section.
%
%\subsection{Polynomial-time algorithms when $h=2$ \yota{and $|C| = n$}}
%\label{sec:h2}
%\input{h2}



% 前の方で O(h^n) で解けることが示されているので，こちらはコメントアウト
%
%\subsection{Polynomial-time algorithm for a fixed $n$}
%\label{sec:fpt}
%\input{fpt}



==> pre.tex <==
In this paper, we investigate the computational complexity of
the ball sort puzzle (BSP) and the water sort puzzle (WSP).
The difference of these puzzles is operations we can use for sorting.
We first introduce the common features for these sort puzzles.

Let $B$ and $C$ be finite sets of \emph{bins} and \emph{colors}, respectively.
The set of sequences of colors of length at most $h$ is denoted by $C^{\le h}$.
A sequence of $c \in C$ of length $l$ is called \emph{monochrome} and denoted by $c^l$.
The empty sequence is denoted as $\emptyseq$, which is, in our terminology, also called monochrome.
The $i$th element of a sequence $\alpha$ is denoted by $\alpha[i]$ for $1 \le i \le |\alpha|$.
The \emph{top color} of $\alpha$ is $\topcolor{\alpha} = \alpha[|\alpha|]$ if $\alpha$ is not empty.
In case $\alpha$ is empty, $\topcolor{\alpha}$ is defined to be $\emptyseq$. 
A \emph{border} in $\alpha$ is a number $i$ such that either $1 \le i < |\alpha|$ and $\alpha[{i}] \neq \alpha[{i+1}]$ or $i=0$, and
the set of borders of $\alpha$ is denoted by $\mcal{D}(\alpha)$.
We count non-trivial borders as $D(S) = \sum_{b\in B}|\mcal{D}(S(b))\setminus\{0\}|$.
For example, in \figurename~\ref{fig:water1}, the values of $D$ are $4,3,3,3$ in (0), (1), (2), (3), respectively.
A \emph{configuration} is a map $S \colon B \to C^{\le h}$.
An instance of the sort puzzle is a configuration $S$ such that $|S(b)| \in \{h,0\}$ for all $b \in B$.
A bin $b$ is \emph{sorted} under $S$ if $S(b) \in \{\emptyseq, c^h\}$ for some $c \in C$. 
A configuration $S$ is \emph{sorted} or \emph{goal} if all bins are sorted under $S$.
Sometimes we identify $b \in B$ with $S(b)$ when $S$ is clear from the context.

Without loss of generality, we assume that each color $c \in C$ occurs exactly $hj$ times for some positive integer $j$ in a configuration $S$
because the puzzle has no solution otherwise. (This implies that $|C|$ is at most $n$.)
When a bin $|S(b)|=h'$ with $0\le h'\le h$, the \emph{margin} of $b$ is defined by $h-h'$.

We now turn to define a move of the sort puzzle. Intuitively, we pick up two bins $b_i$ and $b_j$ from $B$,
and pour the top item(s) from $b_i$ to $b_j$ if $b_j$ is empty or the top item of $b_j$ has the same color.
The quantity of the items are different in the cases of balls and water.
In the ball case, a unit is moved if possible. On the other hand, two or more units of water of the same color
move at once until all units are moved or $b_j$ becomes full. We define more precisely.
A \emph{ball-move} can modify a configuration $S$ into $S'$, denoted as $S \ballmove S'$, if there are $b_i,b_j\in B$ and $c \in C$ such that
$S(b_i)= S'(b_i) \cdot c$, $\topcolor{S(b_j)}\in \{c,\emptyseq\}$, 
$S'(b_j)= S(b_j) \cdot c$, and $S(b)=S'(b)$ for all $b\in B\setminus\{b_i,b_j\}$.
A \emph{water-move} can modify $S$ into $S'$, denoted as $S \watermove S'$, if there are $m \ge 1$, $b_i,b_j\in B$
and $c\in\calC$ such that 
(1) $S(b_i)= S'(b_i)\cdot c^m$, $\topcolor{S(b_j)}\in \{c,\emptyseq\}$, and $S'(b_j)= S(b_j) \cdot c^m$, 
(2) either $\topcolor{S'(b_i)}\neq c$ or $\msize{S'(b_j)}=h$, and
(3) $S(b)=S'(b)$ for all $b\in B\setminus\{b_i,b_j\}$.
Clearly any single water-move can be simulated by $m$ ball-moves.
The reflexive and transitive closures of $\ballmove$ and $\watermove$ are denoted as $\ballmove^*$ and $\watermove^*$, respectively.

The water sort puzzle asks us to sort the $hn$ units of water in $n+k$ bins.
The computational complexity of the water sort puzzle is measured by the number of moves.
For a given initial configuration $S$ of the water sort puzzle,
the \emph{decision} problem asks whether we can transform $S$ to a goal state by a sequence of moving water units or not.
The \emph{shortest path} problem asks, for given a configuration $S$ and an integer $t$, 
whether we can transform $S$ to a goal state by a sequence of length at most $t$.
The \emph{construction} problem requires to output a solution for $S$.


